Anomaly zones for uniformly sampled gene trees under the gene duplication and loss model

Recently, there has been interest in extending long-known results about the multispecies coalescent tree to other models of gene trees. Results about the gene duplication and loss (GDL) tree have mathematical proofs, including species tree identifiability, estimability, and sample complexity of popular algorithms like ASTRAL. Here, this work is continued by characterizing the anomaly zones of uniformly sampled gene trees. The anomaly zone for species trees is the set of parameters where some discordant gene tree occurs with the maximal probability. The detection of anomalous gene trees is an important problem in phylogenomics, as their presence renders effective estimation methods to being positively misleading. Under the multispecies coalescent, anomaly zones are known to exist for rooted species trees with as few as four species. The gene duplication and loss process is a generalization of the generalized linear-birth death process to the rooted species tree, where each edge is treated as a single timeline with exponential-rate duplication and loss. The methods and results come from a detailed probabilistic analysis of trajectories observed from this stochastic process. It is shown that anomaly zones do not exist for rooted GDL balanced trees on four species, but do exist for rooted caterpillar trees, as with the multispecies coalescent.

==> Old_Files/Coalescence_probabilities.tex <==
It remains to consider the relationship of $k_1$ with $k_2$ and $k_3$.

\newpage

Remove Lemma 2? We first prove the following Lemma.

\begin{lemma} \label{lemma:1}
We have $$\PP'_{N_I}(i_a = i_b = i_c) \geq \frac{1}{N_I^2}$$ and $$\PP'_{N_I}(|\{i_a,i_b,i_c\}| = 3) \leq \frac{2}{N_I} \mathbf{1}(N_I \geq 3).$$
\end{lemma}

\begin{proof}

Conditioning on $N_I$, the ancestors of the sampled copies at $I$ are determined uniformly at random.  However, there is dependence between these selections.  From the law of total probability, we condition on the number of descendants at $J$ of each individual at $i$.  Let $(P_i)_{i=1}^{N_I}$ denote these numbers and $(S_i)_{i=1}^{N_I}$ denote the sets of individuals.  The law of total probability implies $$\PP'_{N_I}(i_a = i_b = i_c) = \EE'_{N_I}\left[\PP'_{N_I}(i_a = i_b = i_c | (P_i)_i)\right].$$ Conditioned on $N_J$ and $(P_j)_{j = 1}^{N_I}$, the ancestors at $J$ are determined uniformly at random, but varying $P_j$ gives a weighted distribution for the ancestors at $I$.  The ancestor of $c$ is also independent from those of $a$ and $b$.   We then have \begin{align*}
&\PP'_{N_I}(i_a = i_b = i_c | (P_i)_i) = \EE'_{N_I}\left[\PP'_{N_I}(j_a, j_b \in S_i | (P_i)_i) \frac{P_i}{\sum_{j=1}^{N_I}P_j}\right]
\end{align*} We then bound $\PP'_{N_I}(j_a, j_b \in S_i | (P_i)_i)$.  For this, we condition further on $(M_{i,k})_{i=1, k \in S_i}^{N_I}$, the progeny sizes of the individuals at $J$.  Using independence, we then have \begin{align*}
&\PP'_{N_I}(i_a = i_b = i_c | (P_i)_i) \frac{P_i}{\sum_{j=1}^{N_I}P_j} = \sum_{i=1}^{N_I}\frac{\sum_{k \in S_{i}}M_{i,k}^2}{(\sum_{i=1}^{N_I}\sum_{k \in S_i}M_{i,k})^2} \frac{P_i}{\sum_{j=1}^{N_I}P_j} \\
&\geq \sum_{i=1}^{N_I} \frac{P_i^3}{(\sum_{i=1}^{N_I}P_i)^3},
\end{align*} where the inequality on the right-hand side comes by observing $\sum_{k \in S_i}M_{i,k}^2 \geq P_i$ for all $i$.  The ``cubic mean inequality'' given by $$\left(\frac{1}{N_I}\sum_{i=1}^{N_I}P_i\right)^{1/3} \geq \frac{1}{N_I}\sum_{i=1}^{N_I}P_i$$ then implies  $$\sum_{i=1}^{N_I} \frac{P_i^3}{(\sum_{i=1}^{N_I}P_i)^3} \geq \frac{1}{N_I^2},$$ as required.

For the second part, note that the required probability equals 0 when $N_I < 3$.  Now we find a bound for $N_I \geq 3.$  Observe first that $$\PP'_{N_I}(|\{i_a,i_b,i_c\}| = 3) \leq \PP'_{N_I}(|\{j_a,j_b,j_c\}| = 3).$$ Similar to before, we condition on $(P_i)_{i}$ and $(M_{i,k})_{i,k}$ and use independence to proceed.  We have \begin{align*}
&\PP'_{N_I}(|\{j_a,j_b,j_c\}| = 3) \\
&= \sum_{j \ne j'}\EE'_{N_I}\left[ \EE'_{N_I}\left[\frac{(\sum_{k \in S_j}M_{j,k})(\sum_{k \in S_{j'}}M_{j',k})}{(\sum_{i=1}^{N_I}\sum_{k \in S_i}M_{i,k})^2} \bigg| (M_{i,k}), (P_i)_{i}\right]\left(1 - \frac{P_j+P_{j'}}{\sum_{i=1}^{N_I}P_i}\right)\bigg| (P_i)_{i}\right]
\end{align*} The function $$1 - \frac{P_j + P_{j'}}{\sum_{i=1}^{N_I}P_i}$$ is decreasing in the arguments $P_j$ and $P_{j'}$ but increasing in the other arguments.  Because the $P_j$ are not bounded, we have $$1 - \frac{P_j + P_{j'}}{\sum_{i=1}^{N_I}P_i} = \frac{\sum_{i \ne j,j'}P_{i}}{\sum_{i=1}^{N_I}P_i} \leq \frac{1}{N_I-2}.$$ Bounding this portion, the tower property allows us to factor it out of the expectation.  Using $$\sum_{j \ne j'} \frac{(\sum_{k \in S_j}M_{j,k})(\sum_{k \in S_{j'}}M_{j',k})}{(\sum_{i=1}^{N_I}\sum_{k \in S_i}M_{i,k})^2} = 1 - \sum_{i=1}^{N_I} \frac{(\sum_{k \in S_i}M_{i,k})^2}{(\sum_{i=1}^{N_I}\sum_{k \in S_i}M_{i,k})^2} \leq 1 - \frac{1}{N_I}.$$ Putting it together, we obtain $$\PP'_{N_I}(|\{i_a,i_b,i_c\}| = 3) \leq \left(1 - \frac{1}{N_I}\right)\frac{1}{N_I - 2} \leq \frac{2}{N_I}.$$
\end{proof}

==> Old_Files/J_given_I_conditions.tex <==
\begin{proof}[Proof of Proposition \ref{prop:11}]
There are four cases of events that give the species tree with positive probability.  They are (i) $j_a = j_b = j_c$; (ii) $j_a = j_b \ne j_c$ and $i_a = i_b = i_c$; (iii) $j_a = j_b \ne j_c$, $i_a = i_b \ne i_c$, and $i_d$ is different; and (iv) $j_a,j_b,j_c$ are distinct and $i_a,i_b,i_c,i_d$ are distinct.  We compute the probability of each case and the conditional probability of $(((a,b),c),d)$ given possibility.

\hfill

(i) In the case that $j_a = j_b = j_c$, the required topology occurs with probability $1$.  The probability of $j_a = j_b = j_c$ is characterized by conditioning on $N_J$.  We first have $$
\PP'(j_a = j_b = j_c) = \EE'\left[ \PP'_{N_J}(j_a = j_b = j_c) \right].$$  Conditioned on $N_J$, the choice of $j_c$ is independent of $\{j_a,j_b\}$.  We then have $$
\PP'_{N_J}(j_a = j_b = j_c) = \sum_{k=1}^{N_J} \frac{1}{N_J} \PP'_{N_J}(j_a = j_b = k).$$ Letting $(N_k)_{k=1}^{N_J}$ be the progeny of each individual at $N_J$ surviving to $K$, we have $$\PP'_{N_J}(j_a = j_b = k) = \EE'_{N_J} \left[ \frac{N_k^2}{\left(\sum_{k=1}^{N_J}N_k \right)^2} \bigg| (N_k)_{k=1}^{N_J}\right].$$ Putting it together, we have $$\PP'(j_a = j_b = j_c) = \EE'\left[ \frac{1}{N_J} \EE'_{N_J}\left[ \frac{\sum_{k=1}^{N_J}N_k^2}{\left(\sum_{k=1}^{N_J}N_k\right)^2} \bigg| (N_k)_{k=1}^{N_J} \right]\right].$$

\hfill

(ii) In the case that $j_a = j_b \ne j_c$ and $i_a = i_b = i_c$, the required topology occurs with probability $1$.  We start by conditioning on $N_I$, i.e. $$\PP'(j_a = j_b \ne j_c, i_a = i_b = i_c) = \EE'\left[\PP'_{N_I}(j_a = j_b \ne j_c, i_a = i_b = i_c)\right].$$ Conditioned on $N_I$, the progenies at $I$ are exchangeable, so \begin{align*}
&\EE'\left[\PP'_{N_I}(j_a = j_b \ne j_c, i_a = i_b = i_c)\right] = \EE'\left[N_I \PP'_{N_I}(j_a = j_b \ne j_c, i_a = i_b = i_c = i)\right] \\
&= \EE'\left[N_I \PP'_{N_I}(j_a = j_b \ne j_c|i_a = i_b = i_c = i)\PP'_{N_I}(i_a = i_b = i_c = i)\right] \\
&= \EE'\left[N_I \PP'_{N_I = 1}(j_a = j_b \ne j_c)\PP'_{N_I}(i_a = i_b = i_c = 1)\right].
\end{align*} On the right-hand side, we let $\PP'_{N_I = 1}$ denote the measure conditioned on $N_I = 1$ and used independence of the progenies of individuals at $I$.  Now, we proceed inductively.  Let $\PP'_{N_I = 1,N_J}$ denote the measure conditioned on $N_I = 1$ and $N_J$.  Then \begin{align*}\PP'_{N_I = 1}(j_a = j_b \ne j_c) &= \EE'_{N_I = 1} \left[\PP'_{N_I = 1,N_J}(j_a = j_b \ne j_c)\right] \\
&= \EE'_{N_I = 1} \left[ \EE'_{N_I = 1,N_J} \left[\left(1 - \frac{1}{N_J}\right) \frac{\sum_{j=1}^{N_J}N_j^2}{\left(\sum_{j=1}^{N_J}N_j\right)^2} \bigg| (N_j)_{j=1}^{N_J}\right]\right] .
\end{align*} (We will quantify $\PP'_{N_I}(i_a = i_b = i_c = 1)$ and related probabilities later.)

\hfill

(iii) In the case that $j_a = j_b \ne j_c$ and $i_a = i_b \ne i_c$ and $i_d$ is different from $i_a$ and $i_c$, the required topology occurs with probability $1/3$.  This is because there are three possibilities between $i_a,i_c,i_d$ for who are siblings in the stem edge, and all arrangements are equally likely.  As with part (ii), we condition on $N_I$:  $$\PP'(j_a = j_b \ne j_c, |\{i_{a},i_c,i_d\}| = 3) = \EE'\left[\PP'_{N_I}(j_a = j_b \ne j_c, |\{i_{a},i_c,i_d\}| = 3)\right].$$  Using exchangeability, the right-hand side equals 
$$\EE'\left[ \left(1 - \frac{2}{N_I}\right) \begin{pmatrix}
N_I \\
2
\end{pmatrix} \PP'_{N_I}(j_a = j_b \ne j_c| i_a = i_b = 1, i_c = 2) \PP'_{N_I}(i_a = i_b = 1, i_c = 2)\right].$$
